vid-TLDR: Training Free Token merging for Light-weight Video Transformer

Video Transformers have become the prevalent solution for various video downstream tasks with superior expressive power and flexibility. However, these video transformers suffer from heavy computational costs induced by the massive number of tokens across the entire video frames, which has been the major barrier to training the model. Further, the patches irrelevant to the main contents, e.g., backgrounds, degrade the generalization performance of models. To tackle these issues, we propose training free token merging for lightweight video Transformer (vid-TLDR) that aims to enhance the efficiency of video Transformers by merging the background tokens without additional training. For vid-TLDR, we introduce a novel approach to capture the salient regions in videos only with the attention map. Further, we introduce the saliency-aware token merging strategy by dropping the background tokens and sharpening the object scores. Our experiments show that vid-TLDR significantly mitigates the computational complexity of video Transformers while achieving competitive performance compared to the base model without vid-TLDR. Code is available at https://github.com/mlvlab/vid-TLDR.

==> Main/preamble.tex <==
%
% --- inline annotations
%
% \usepackage{hyperref}
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}

% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}

\usepackage{url}

\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{colortbl}         % colors

\usepackage{graphicx}
\usepackage{multirow}
\usepackage{amsmath}
\usepackage{subcaption}
\usepackage{graphicx}
\usepackage{algorithm}
\usepackage{algpseudocode}

% \newcommand{\green}[1]{{\color{green}#1}}
% \newcommand{\green}{\textcolor[rgb]{0.8,0.9,0.1}}
\newcommand{\cyan}[1]{{\color{Cyan}#1}}
\newcommand{\green}{\textcolor[rgb]{0.1,0.9,0.1}}
\newcommand{\gray}{\textcolor[rgb]{0.5,0.5,0.5}}
% \newcommand{\red}{\textcolor[rgb]{1,0,0}}
\newcommand{\blue}{\textcolor[rgb]{0,0,1}}
\newcommand{\yellow}{\textcolor[rgb]{1,1,0.8}}
\newcommand{\orange}{\textcolor[rgb]{1,0.48,0.05}}
\newcommand{\sh}{\textcolor[rgb]{1,0,1}}


% \crefname{section}{Sec.}{Secs.}
% \crefname{appendix}{Sec.}{Secs.}
% \crefname{table}{Tab.}{Tabs.}
% \crefname{figure}{Fig.}{Figs.}
% \crefname{equation}{Eq.}{Eqs.}

% \Crefname{section}{Section}{Sections}
% \Crefname{appendix}{Section}{Sections}
% \Crefname{table}{Table}{Tables}
% \Crefname{figure}{Figure}{Figures}
% \Crefname{equation}{Equation}{Equations}


\definecolor{Gray}{rgb}{0.8,0.8,0.8} %255 204 204
\definecolor{LightBlue}{rgb}{0.8,0.9,1} %204 229 255
\definecolor{LightOrange}{rgb}{1,0.9,0.8} %255 229 204
\definecolor{Cyan}{rgb}{0,1,1} 

\newtheorem{theorem}{Theorem}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{remark}{Remark}

\makeatletter
\def\thickhline{%
  \noalign{\ifnum0=`}\fi\hrule \@height \thickarrayrulewidth \futurelet
   \reserved@a\@xthickhline}
\def\@xthickhline{\ifx\reserved@a\thickhline
               \vskip\doublerulesep
               \vskip-\thickarrayrulewidth
             \fi
      \ifnum0=`{\fi}}
\makeatother

\newlength{\thickarrayrulewidth}
\setlength{\thickarrayrulewidth}{3\arrayrulewidth}

==> Supple/zero_shot_all.tex <==
\begin{table*}[ht]
\centering
\vspace{-8pt}
\caption{
    \textbf{Comparison of zero-shot retrieval results among a baseline model~\cite{li2023unmasked}, existing token merging method (ToMe~\cite{bolya2022token}) and ours}.    
}
\vspace{-7pt}
\label{sup:zero-shot-all}
\begin{tabular}{c|c|ccc|ccc}
\thickhline

\multirow{2}{*}{} & \multirow{2}{*}{Metic} &  \multicolumn{3}{c|}{UMT-B} & \multicolumn{3}{c}{UMT-L} \\
 & & \multicolumn{1}{c}{Base} & \multicolumn{1}{c}{ToMe} & \multicolumn{1}{c|}{Ours} & \multicolumn{1}{c}{Base} & \multicolumn{1}{c}{ToMe} & \multicolumn{1}{c}{Ours} \\ \hline
 \multirow{4}{*}{Average over 4 datasets}  & GFLOPs $\downarrow$ & 78.5 & 64.7 & \textbf{48.5} & 267.8 & 179.9 & \textbf{158.7} \\
 \cline{2-8}
  & R@1  $\uparrow$ & 36.9 & 35.1 (\blue{-1.5}) & \textbf{38.0} (\red{+1.1})  & 43.7 & 42.2 (\blue{-1.5}) & \textbf{44.4} (\red{+0.7}) \\ 
  & R@5  $\uparrow$ & 61.0 & 59.2 (\blue{-1.8}) & \textbf{62.0} (\red{+1.0}) & 67.9 & 66.7 (\blue{-0.8}) & \textbf{68.4} (\red{+0.5}) \\ 
  & R@10 $\uparrow$ & 67.4 & 65.7 (\blue{-1.7}) & \textbf{68.3} (\red{+0.9}) & 73.6 & 72.6 (\blue{-1.0}) & \textbf{74.0} (\red{+0.4}) \\
  
\thickhline

\end{tabular}
\end{table*}



==> Tables/retrieval_old.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

% \def\arraystretch{1.2}
\begin{table}[t!]
\centering
\resizebox{\pagewidth}{!}{
\begin{tabular}{l|r|ccc|ccc|ccc|ccc}
\thickhline
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Method}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\#Pairs}}} & \multicolumn{3}{c|}{\textbf{MSRVTT}} & \multicolumn{3}{c|}{\textbf{DiDeMo}} & \multicolumn{3}{c}{\textbf{ActivityNet}} \\
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{}                                & R@1        & R@5        & R@10       & R@1     & R@5     & R@10    & R@1       & R@5      & R@10     \\ \hline
ClipBERT~\cite{lei2021less}                                              & 5.4M  & 22.0       & 46.8       & 59.9       & 20.4    & 48.0    & 60.8    & 21.3      & 49.0     & 63.5     \\
Frozen~\cite{Bain21}                                                & 5M  & 31.0       & 59.5       & 70.5       & 34.6    & 65.0    & 74.7    & \multicolumn{3}{c}{-}           \\
VIOLET~\cite{fu2021violet}                                                & 138M  & 34.5       & 63.0       & 73.4       & 32.6    & 62.8    & 74.7    & \multicolumn{3}{c}{-}           \\
All-in-one~\cite{jinpeng2022all}                                            & 138M & 37.9       & 68.1       & 77.1       & 32.7    & 61.4    & 73.5    & 22.4      & 53.7     & 67.7     \\
LAVENDER~\cite{li2023lavender}                                              & 30M  & 40.7       & 66.9       & 77.6       & 53.4    & 78.6    & 85.3    & \multicolumn{3}{c}{-}           \\
Singularity~\cite{lei2022revealing}                                           & 17M  & 42.7       & 69.5       & 78.1       & 53.1    & 79.9    & 88.1    & 48.9      & 77.0     & 86.3     \\
OmniVL~\cite{wang2022omnivl}                                                & 17M & 47.8       & 74.2       & 83.8       & 52.4    & 79.5    & 85.4    & \multicolumn{3}{c}{-}           \\
VINDLU~\cite{cheng2023vindlu}                                                & 25M & 46.5       & 71.5       & 80.4       & 61.2    & 85.8    & 91.0    & 55.0      & 81.4     & 89.7     \\
CLIP4Clip~\cite{luo2022clip4clip}                                             & 400M & 44.5       & 71.4       & 81.6       & 42.8    & 68.5    & 79.2    & 40.5      & 72.4     & 83.4     \\
CLIP-ViP~\cite{xue2022clip}                                              & 500M  & 54.2       & 77.2       & 84.8       & 50.5    & 78.4    & 87.1    & 53.4      & 81.4     & 90.0     \\
InternVideo~\cite{wang2022internvideo}                                           & 646M  & 55.2       & 79.6       & 87.5       & 57.9    & 82.4    & 88.9    & 62.2      & 85.9     & 93.2     \\ \hline
UMT-B~\cite{li2023unmasked}                                                 & 25M    & 51.0       & 76.5       & 84.2       & 61.6    & 86.8    & 91.5    & 58.3      & 83.9     & 91.5     \\
UMT-L~\cite{li2023unmasked}                                                 & 25M  & 58.8       & 81.0       & 87.1       & 70.4    & 90.1    & 93.5    & 66.8      & 89.1     & 94.9     \\ \hline
UMT-B-Ours                                            & 25M  & 51.3       & 00.0       & 00.0       & 63.1    & 00.0    & 00.0    & 57.7      & 00.0     & 00.0     \\
UMT-L-Ours                                            & 25M & 58.2       & 00.0       & 00.0       & 69.8    & 00.0    & 00.0    & 66.3      & 00.0     & 00.0     \\ \thickhline
\end{tabular}
}
\caption{
    Text-to-video retrieval on MSRVTT, DiDeMo, AcitivityNet. “\#Pairs” denotes the number of pre-training pairs.
}
\label{table:retrieval2}
\end{table}


% \label{table:retrieval}
% \caption{
%     Text-to-video retrieval on MSRVTT, DiDeMo, AcitivityNet. “\#Pairs” denotes the number of pre-training pairs.
% }

==> rebuttal/tab_other1.tex <==
\begin{table}[h!]
\vspace{-10pt}
\small
  \centering 
  \caption{Action recognition with VideoMAE on UCF101 \& Something Something V2.}
\vspace{-10pt}
  \label{tab:other1}
    \centering
    \setlength{\tabcolsep}{2pt}
    \resizebox{\linewidth}{!}{\begin{tabular}{l|llll}
         &  \multicolumn{2}{c}{UCF101} & \multicolumn{2}{c}{SSv2}  \\
         & \multicolumn{1}{c}{FLOPs} & \multicolumn{1}{c}{Acc} & \multicolumn{1}{c}{FLOPs} & \multicolumn{1}{c}{Acc}\\
        \midrule
        VideoMAE & 180.5  & 91.3 & 180.5 & 70.8 \\
        +ToMe& 58.4 \scriptsize(-67.6\%) & 75.7 \scriptsize(-15.6) & 58.4 \scriptsize(-67.6\%) & 58.5 \scriptsize(-12.3)  \\
        +vid-TLDR & 56.1 \scriptsize(-68.8\%) & 90.1 \scriptsize(-1.2) & 56.6  \scriptsize(-68.6\%) & 69.6 \scriptsize(-1.2)\\
  \end{tabular}}
\vspace{-10pt}
\end{table}

==> rebuttal/tab_other2.tex <==
\begin{table}[h!]
\vspace{-10pt}
\small
  \centering 
  \caption{Base-to-novel generalization. HM : Harmonic mean}
\vspace{-10pt}
  \label{tab:other2}
    \centering
    \setlength{\tabcolsep}{2pt}
    \resizebox{\linewidth}{!}{\begin{tabular}{l|llll}
        UCF101 & \multicolumn{1}{c}{FLOPs} & \multicolumn{1}{c}{Base} & \multicolumn{1}{c}{Novel} & \multicolumn{1}{c}{HM}\\
        \midrule
        ViFi-CLIP & 563  & 92.9 & 67.7 & 78.3 \\
        +ToMe& 279 \scriptsize(-50.4\%) & 72.0 \scriptsize(-20.9)  & 44.8 \scriptsize(-22.9) & 55.3 \scriptsize(-23.0) \\
        +vid-TLDR & 279 \scriptsize(-50.4\%) & 91.3 \scriptsize(-1.6) & 63.2 \scriptsize(-4.5) & 74.7 \scriptsize(-3.6)\\
  \end{tabular}}
\vspace{-10pt}
\end{table}

==> rebuttal/tab_sensitivity.tex <==
\begin{table}[t!]
% \vspace{-10pt}
\small
  \centering 
  \caption{Sensitivity analysis of vid-TLDR on more layers.}
\vspace{-10pt}
  \label{tab:abl}
    \centering
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}{c|cccc}
        layers / $r$ & FLOPs & T2V & V2T & Mean\\
        \midrule
        - / 0  & 303.3 & 51 & 49.0 & 50.0\\
        \midrule
        (1-2) / 450 & 178.4 & 51.0 & 49.9 & 50.5\\
        (1-4) / 225 & 190.9 & 50.5 & 49.4 & 50.0\\
        (1-6) / 150 & 203.6 & 50.2 & 49.4 & 49.8\\
        (1-8) / 112 & 216.4 & 49.7 & 49.2 & 49.5\\
        (1-10) / 90 & 228.8 & 48.7 & 48.0 & 48.35\\
        (1-12) / 75 & 241.4 & 47.6 & 48.4 & 48.0\\
  \end{tabular}
\vspace{-20pt}
\end{table}
